Millimeter-Wave Path Loss at 73 GHz in Indoor and Outdoor Airport Environments

In this paper, two large-scale fading path loss models are presented based on indoor and outdoor channel measurements at 73 GHz. The line-of-sight millimeter-wave propagation measurement campaigns were uniquely conducted within the indoor and outdoor environments at an airport setting, i.e., the Boise Airport. The channel measurements were made with directional transmit and receive antennas with a 24 dBi gain at different receive antenna heights. From the measured data, we obtained the parameters of two path loss models, i.e., the close-in reference distance model (CIM) and the floating-intercept model (FIM). Results show that the path loss exponents estimated from the CIM are very close to that of the free-space path loss model, while the FIM provides a better fit to the measurement data.

==> ref <==
@book{rappaport1996wireless,
  title={Wireless communications: principles and practice},
  author={Rappaport, Theodore S and others},
  volume={2},
  year={1996},
  publisher={prentice hall PTR New Jersey}
}


@book{rappaport2014millimeter,
  title={Millimeter wave wireless communications},
  author={Rappaport, Theodore S and Heath Jr, Robert W and Daniels, Robert C and Murdock, James N},
  year={2014},
  publisher={Pearson Education}
}


@misc{nyusim,
    title={NYUSIM {5G} Channel Simulator },
    url={https://wireless.engineering.nyu.edu/nyusim-5{G}-channel-simulator-now-available/},
    urldate={2016-07-13},
    }

@inproceedings{maccartney2014omnidirectional,
  title={Omnidirectional path loss models in {New} {York} {City} at 28{ GHz} and 73 {GHz}},
  author={MacCartney, George R and Samimi, Mathew K and Rappaport, Theodore S},
  booktitle={IEEE Int. Symposium},
  pages={227--231},
  year={2014},
  organization={IEEE}
}

@inproceedings{samimi20153,
  title={3-{D} statistical channel model for millimeter-wave outdoor mobile broadband communications},
  author={Samimi, Mathew K and Rappaport, Theodore S},
  booktitle={ IEEE ICC},
  pages={2430--2436},
  year={2015},
  organization={IEEE}
}
@article{rappaport2015wideband,
  title={Wideband millimeter-wave propagation measurements and channel models for future wireless communication system design},
  author={Rappaport, Theodore S and MacCartney, George R and Samimi, Mathew K and Sun, Shu},
  journal={IEEE Trans. on Communications},
  volume={63},
  number={9},
  pages={3029--3056},
  year={2015},
  publisher={IEEE}
}

@ARTICLE{1296643, 
author={C. R. Anderson and T. S. Rappaport}, 
journal=IEEE_M_WC, 
title={In-building wideband partition loss measurements at 2.5 and 60 {GHz}}, 
year={2004}, 
volume={3}, 
number={3}, 
pages={922-928}, 
ISSN={1536-1276}, 
month={May},}

@article{rangan2014millimeter,
  title={Millimeter-wave cellular wireless networks: Potentials and challenges},
  author={Rangan, Sundeep and Rappaport, Theodore S and Erkip, Elza},
  journal={ IEEE Proceed.},
  volume={102},
  number={3},
  pages={366--385},
  year={2014},
  publisher={IEEE}
}

@ARTICLE{rqppaport2013Itwillwork, 
author={T. S. Rappaport and S. Sun and R. Mayzus and H. Zhao and Y. Azar and K. Wang and G. N. Wong and J. K. Schulz and M. Samimi and F. Gutierrez}, 
journal={IEEE Access}, 
title={Millimeter Wave Mobile Communications for 5{G }Cellular: It Will Work!}, 
year={2013}, 
volume={1}, 
number={}, 
pages={335-349}, 
ISSN={2169-3536}, 
month={},}




@inproceedings{rappaport201238,
  title={38{GHz} and 60 {GHz} angle-dependent propagation for cellular \& peer-to-peer wireless communications.},
  author={Rappaport, Theodore S and Ben-Dor, Eshar and Murdock, James and Qiao, Yijun},
  booktitle={Proc. IEEE ICC},
  pages={4568--4573},
  year={Jun. 2012}
    }
    
    
  @article{azar2013,
   author={Azar, Yaniv},
   title={28{ GHz} propagation measurements for outdoor cellular communications using steerable beam antennas in New York City},
   journal={Proc. IEEE ICC},
   pages={5143--5147},
  year={Jun 2013},
  organization={}
 
}


@article{kyosti2007winner,
  title={WINNER {II} channel models},
  author={Kyosti, Pekka},
  journal={Eur. Commission,Brussels},
  year={ Belgium, IST-WINNER, Tech. Rep. D1.1.2}
}


  @article{GPP,
   author={},
   title={Spatial channel model for multiple input multiple output
{(MIMO)} simulations},
   journal={3rd Generation Partnership Project, Sophia
Antipolis Cedex},
   pages={},
  year={ France, TR 25.996, Sep. 2003},
  organization={}
 
}



@article{mahfuza2017,
   author={Khatun, Mahfuza and Mehrpouyan, Hani and Matolak, David and Guvenc, Ismail},
   title={Millimeter Wave Systems for Airports and Short-Range Aviation Communications: A Survey of the Current Channel Models at mmWave Frequencies},
   journal={IEEE Digital Avia. Systems Conf.},
   year=2017,
 
}


@inproceedings{maccartney2013path,
  title={Path loss models for {5G} millimeter wave propagation channels in urban microcells},
  author={MacCartney, George R and Zhang, Junhong and Nie, Shuai and Rappaport, Theodore S},
  booktitle={IEEE Glob. Comm. Conf.},
  pages={3948--3953},
  year={2013},

}
@article{mahfuza2018,
   author={Khatun, M. and Mehrpouyan, H. and Matolak, D.},
   title={60-{GHz} Millimeter-Wave Pathloss Measurements in Boise Airport},
   journal={IEEE Glob. Conf. on Signal and Inform. Process.},
  pages={1276--1280},
  year={2018},
  publisher={}
}
@inproceedings{zhang2004solving,
  title={Solving large scale linear prediction problems using stochastic gradient descent algorithms},
  author={Zhang, Tong},
  booktitle={Proceed. of the twenty-first int. conf. on Machine learning},
  pages={116},
  year={2004},
  organization={ACM}
}


@article{shad2019,
   author={Shad, S. and Mehrpouyan, H},
   title={A Dielectric-Loaded Waveguide Aperture Antenna Based on Waveguide-Fed Cavity-Backed in the 60-{GHz} Band},
   journal={IEEE Texas Sympo. on Wireless and Micro. Circuuit and Sys.},
  pages={1--4},
  year={2019},
 publisher={}
 }
 @article{almasi2019lens,
  title={Lens-based Millimeter Wave Reconfigurable Antenna NOMA},
  author={Almasi, Mojtaba Ahmadi and Amiri, Roohollah and Vaezi, Mojtaba and Mehrpouyan, Hani},
  journal={IEEE International Conf. on Commun. Workshops},
  pages={1--5},
  year={2019}
}
